Probing scattering of Raman phonons on magnetic and electronic excitations in pyrochlores Nd$_2$Zr$_2$O$_7$ and Nd$_2$Ir$_2$O$_7$

Magnetic rare earth atoms on pyrochlore lattice can produce such exotic magnetic states as spin ice and quantum spin ice. These states are a result of the frustration in the pyrochlore lattice, as well as crystal field degrees of freedom of rare earth atoms, and their interactions with the lattice. Raman scattering spectroscopy, which possess high spectral resolution and can easily access broad energy and temperature ranges, is an optimum tool to study these excitations and their interactions. In this work we follow Raman scattering of zone center phonons and crystal field excitations of Nd$^{3+}$ in Nd$_2$Zr$_2$O$_7$ and Nd$_2$Ir$_2$O$_7$ in the temperature range where these materials are paramagnetic. A comparison between an insulating Nd$_2$Zr$_2$O$_7$ and semimetallic Nd$_2$Ir$_2$O$_7$ materials allow us to distinguish between scattering of phonons on other phonons, crystal field excitations, and electrons, highlighting interactions between these degrees of freedom.

==> CoverLetter.tex <==
Dear Editor,

Please find enclosed our manuscript "Scattering of Raman  phonons on magnetic and electronic excitations in  pyrochlores Nd$_2$Zr$_2$O$_7$ and Nd$_2$Ir$_2$O$_7$." by S. Muhammad et al. Nd-based pyrochlores discussed in this paper attracted a lot of attention of the community working in frustrated magnetism, topology, and electronic correlations due to low temperature exotic magnetism (quantum spin ice state in Nd$_2$Zr$_2$O$_7$) and electronic topological properties (Weyl semimetal state in Nd$_2$Ir$_2$O$_7$). Our work presented in this manuscript probes coupling of  magnetic and electronic degrees of freedom to the lattice in these materials in the paramagnetic state,  at temperatures above the ground states typically discussed. We find that a comparison of these two materials, which have very similar crystal structure and Nd magnetic sublattice, but very different electronic properties due to Zr/Ir sublattice  provides an important insight into understanding of competing interactions in pyrochlores with exotic magnetic and electronic properties. We expect it to be of interest to a broad scope of readers of Phys. Rev. B

With best regards,
On behalf of the authors of the manusctript,
Sami Muhammad, Natalia Drichko
